Constrained Detecting Arrays: Mathematical Structures for Fault Identification in Combinatorial Interaction Testing

Context: Detecting arrays are mathematical structures aimed at fault identification in combinatorial interaction testing. However, they cannot be directly applied to systems that have constraints among test parameters. Such constraints are prevalent in real-world systems. Objectives: This paper proposes Constrained Detecting Arrays (CDAs), an extension of detecting arrays, which can be used for systems with constraints. Methods: The paper examines the properties and capabilities of CDAs with rigorous arguments. The paper also proposes two algorithms for constructing CDAs: One is aimed at generating minimum CDAs and the other is a heuristic algorithm aimed at fast generation of CDAs. The algorithms are evaluated through experiments using a benchmark dataset. Results: Experimental results show that the first algorithm can generate minimum CDAs if a sufficiently long generation time is allowed, and the second algorithm can generate minimum or near-minimum CDAs in a reasonable time. Conclusion: CDAs enhance detecting arrays to be applied to systems with constraints. The two proposed algorithms have different advantages with respect to the array size and generation time

==> 12cdaWithResultsCase2.tex <==
\begin{tabular}{c|cccccc}
\cline{1-5} \cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} \cline{7-7} 
 & $F_1$ & $F_2$ & $F_3$ & $F_4$ &  & Result\tabularnewline
\cline{1-5} \cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} \cline{7-7} 
$\boldsymbol\sigma_1$ & 0 & 0 & 0 & 0 &  & \textbf{Fail}\tabularnewline
$\boldsymbol\sigma_2$ & 0 & 0 & 0 & 1 &  & \textbf{Fail}\tabularnewline
$\boldsymbol\sigma_3$ & 0 & 0 & 0 & 3 &  & \textbf{Fail}\tabularnewline
$\boldsymbol\sigma_4$ & 0 & 0 & 1 & 1 &  & \textbf{Fail}\tabularnewline
$\boldsymbol\sigma_5$ & 0 & 0 & 2 & 2 &  & Pass\tabularnewline
$\boldsymbol\sigma_6$ & 0 & 1 & 1 & 2 &  & Pass\tabularnewline
$\boldsymbol\sigma_7$ & 0 & 1 & 2 & 0 &  & Pass\tabularnewline
$\boldsymbol\sigma_8$ & 0 & 1 & 2 & 1 &  & \textbf{Fail}\tabularnewline
$\boldsymbol\sigma_9$ & 1 & 0 & 0 & 2 &  & Pass\tabularnewline
$\boldsymbol\sigma_{10}$ & 1 & 0 & 0 & 3 &  & Pass\tabularnewline
$\boldsymbol\sigma_{11}$ & 1 & 0 & 1 & 0 &  & Pass\tabularnewline
$\boldsymbol\sigma_{12}$ & 1 & 0 & 2 & 1 &  & Pass\tabularnewline
$\boldsymbol\sigma_{13}$ & 1 & 1 & 1 & 1 &  & Pass\tabularnewline
$\boldsymbol\sigma_{14}$ & 1 & 1 & 2 & 0 &  & Pass\tabularnewline
$\boldsymbol\sigma_{15}$ & 1 & 1 & 2 & 2 &  & Pass\tabularnewline
$\boldsymbol\sigma_{16}$ & 2 & 0 & 0 & 0 &  & Pass\tabularnewline
$\boldsymbol\sigma_{17}$ & 2 & 0 & 0 & 1 &  & Pass\tabularnewline
$\boldsymbol\sigma_{18}$ & 2 & 0 & 0 & 2 &  & Pass\tabularnewline
$\boldsymbol\sigma_{19}$ & 2 & 0 & 0 & 3 &  & Pass\tabularnewline
$\boldsymbol\sigma_{20}$ & 2 & 0 & 1 & 2 &  & Pass\tabularnewline
$\boldsymbol\sigma_{21}$ & 2 & 0 & 2 & 0 &  & Pass\tabularnewline
$\boldsymbol\sigma_{22}$ & 2 & 1 & 1 & 0 &  & Pass\tabularnewline
$\boldsymbol\sigma_{23}$ & 2 & 1 & 1 & 1 &  & Pass\tabularnewline
$\boldsymbol\sigma_{24}$ & 2 & 1 & 2 & 2 &  & Pass\tabularnewline
\cline{1-5} \cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} \cline{7-7} 
\end{tabular}


==> 12claWithResultsCase2.tex <==
\begin{tabular}{c|cccccc}
\cline{1-5} \cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} \cline{7-7} 
 & $F_1$ & $F_2$ & $F_3$ & $F_4$ &  & Result\tabularnewline
\cline{1-5} \cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} \cline{7-7} 
$\boldsymbol\sigma_1$ & 0 & 0 & 0 & 0 &  & \textbf{Fail}\tabularnewline
$\boldsymbol\sigma_2$ & 0 & 0 & 0 & 3 &  & \textbf{Fail}\tabularnewline
$\boldsymbol\sigma_3$ & 0 & 0 & 1 & 1 &  & \textbf{Fail}\tabularnewline
$\boldsymbol\sigma_4$ & 0 & 1 & 1 & 2 &  & Pass\tabularnewline
$\boldsymbol\sigma_5$ & 0 & 1 & 2 & 0 &  & Pass\tabularnewline
$\boldsymbol\sigma_6$ & 1 & 0 & 0 & 2 &  & Pass\tabularnewline
$\boldsymbol\sigma_7$ & 1 & 0 & 0 & 3 &  & Pass\tabularnewline
$\boldsymbol\sigma_8$ & 1 & 0 & 1 & 2 &  & Pass\tabularnewline
$\boldsymbol\sigma_9$ & 1 & 1 & 1 & 1 &  & Pass\tabularnewline
$\boldsymbol\sigma_{10}$ & 1 & 1 & 2 & 0 &  & Pass\tabularnewline
$\boldsymbol\sigma_{11}$ & 1 & 1 & 2 & 2 &  & Pass\tabularnewline
$\boldsymbol\sigma_{12}$ & 2 & 0 & 0 & 1 &  & Pass\tabularnewline
$\boldsymbol\sigma_{13}$ & 2 & 0 & 0 & 3 &  & Pass\tabularnewline
$\boldsymbol\sigma_{14}$ & 2 & 0 & 2 & 0 &  & Pass\tabularnewline
$\boldsymbol\sigma_{15}$ & 2 & 1 & 1 & 0 &  & Pass\tabularnewline
$\boldsymbol\sigma_{16}$ & 2 & 1 & 1 & 2 &  & Pass\tabularnewline
$\boldsymbol\sigma_{17}$ & 2 & 1 & 2 & 1 &  & Pass\tabularnewline
\cline{1-5} \cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} \cline{7-7} 
\end{tabular}


==> 2ccaWithResultsCase2.tex <==
\begin{tabular}{c|cccccc}
\cline{1-5} \cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} \cline{7-7} 
 & $F_1$ & $F_2$ & $F_3$ & $F_4$ &  & Result\tabularnewline
\cline{1-5} \cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} \cline{7-7} 
$\boldsymbol\sigma_1$ & 0 & 0 & 0 & 0 &  & \textbf{Fail}\tabularnewline
$\boldsymbol\sigma_2$ & 0 & 0 & 0 & 3 &  & \textbf{Fail}\tabularnewline
$\boldsymbol\sigma_3$ & 0 & 1 & 1 & 1 &  & \textbf{Fail}\tabularnewline
$\boldsymbol\sigma_4$ & 0 & 1 & 2 & 2 &  & Pass\tabularnewline
$\boldsymbol\sigma_5$ & 1 & 0 & 0 & 2 &  & Pass\tabularnewline
$\boldsymbol\sigma_6$ & 1 & 0 & 0 & 3 &  & Pass\tabularnewline
$\boldsymbol\sigma_7$ & 1 & 0 & 2 & 1 &  & Pass\tabularnewline
$\boldsymbol\sigma_8$ & 1 & 1 & 1 & 0 &  & Pass\tabularnewline
$\boldsymbol\sigma_9$ & 2 & 0 & 0 & 1 &  & Pass\tabularnewline
$\boldsymbol\sigma_{10}$ & 2 & 0 & 0 & 3 &  & Pass\tabularnewline
$\boldsymbol\sigma_{11}$ & 2 & 0 & 1 & 2 &  & Pass\tabularnewline
$\boldsymbol\sigma_{12}$ & 2 & 1 & 2 & 0 &  & Pass\tabularnewline
\cline{1-5} \cline{2-5} \cline{3-5} \cline{4-5} \cline{5-5} \cline{7-7} 
\end{tabular}


==> results.tex <==
\begin{tabular}{c|cccccc|cccccc}
\hline 
\multirow{3}{*}{ID} & \multicolumn{6}{c|}{Time (second)} & \multicolumn{6}{c}{Size}\tabularnewline
\cline{2-13} \cline{3-13} \cline{4-13} \cline{5-13} \cline{6-13} \cline{7-13} \cline{8-13} \cline{9-13} \cline{10-13} \cline{11-13} \cline{12-13} \cline{13-13} 
 & \multicolumn{3}{c}{SMT} & \multicolumn{3}{c|}{Two-step} & \multicolumn{3}{c}{SMT} & \multicolumn{3}{c}{Two-step}\tabularnewline
\cline{2-13} \cline{3-13} \cline{4-13} \cline{5-13} \cline{6-13} \cline{7-13} \cline{8-13} \cline{9-13} \cline{10-13} \cline{11-13} \cline{12-13} \cline{13-13} 
 & max & min & avg & max & min & avg & max & min & avg & max & min & avg\tabularnewline
\hline 
1 & 178.33 & 173.52 & 175.27 & 0.13 & 0.09 & 0.11 & 12 & 12 & 12 & 12 & 12 & 12\tabularnewline
2 & \textbf{1,394.04} & \textbf{979.46} & \textbf{1,067.63} & 0.33 & 0.31 & 0.32 & \textbf{26} & \textbf{26} & \textbf{26} & 26 & 26 & 26\tabularnewline
3 & \textbf{1,060.41} & \textbf{532.19} & \textbf{867.01} & 0.31 & 0.26 & 0.28 & \textbf{28} & \textbf{28} & \textbf{28} & 32 & 30 & 30.80\tabularnewline
4 & \textbf{402.45} & \textbf{247.70} & \textbf{312.10} & 0.16 & 0.13 & 0.14 & \textbf{14} & \textbf{14} & \textbf{14} & 20 & 19 & 19.20\tabularnewline
5 & \textbf{567.49} & \textbf{556.83} & \textbf{560.27} & 0.29 & 0.28 & 0.28 & \textbf{18} & \textbf{18} & \textbf{18} & 18 & 18 & 18\tabularnewline
6 & 93.22 & 67.39 & 75.93 & 0.13 & 0.11 & 0.12 & 10 & 10 & 10 & 14 & 10 & 11.80\tabularnewline
7 & \textbf{1,792.55} & \textbf{1,446.73} & \textbf{1,530.96} & 0.67 & 0.54 & 0.60 & \textbf{44} & \textbf{43} & \textbf{43.80} & 39 & 38 & 38.20\tabularnewline
\hline 
8 & \textbf{1,708.45} & \textbf{1,344.80} & \textbf{1,465.38} & 0.12 & 0.11 & 0.11 & \textbf{24} & \textbf{24} & \textbf{24} & 37 & 33 & 35.80\tabularnewline
9 & -- -- & -- -- & -- -- & 0.27 & 0.24 & 0.25 & -- -- & -- -- & -- -- & 42 & 39 & 41\tabularnewline
10 & \textbf{1,191.70} & \textbf{1,165.48} & \textbf{1,178.59} & 0.30 & 0.24 & 0.26 & \textbf{54} & \textbf{54} & \textbf{54} & 50 & 49 & 49.80\tabularnewline
11 & 0.64 & 0.62 & 0.63 & 0.07 & 0.06 & 0.06 & 8 & 8 & 8 & 8 & 8 & 8\tabularnewline
12 & -- -- & -- -- & -- -- & 0.50 & 0.44 & 0.46 & -- -- & -- -- & -- -- & 99 & 95 & 97\tabularnewline
13 & -- -- & -- -- & -- -- & 0.57 & 0.50 & 0.53 & -- -- & -- -- & -- -- & 61 & 56 & 58.8\tabularnewline
14 & -- -- & -- -- & -- -- & 44.27 & 41.83 & 42.78 & -- -- & -- -- & -- -- & 192 & 180 & 184.20\tabularnewline
15 & -- -- & -- -- & -- -- & 268.53 & 252.81 & 262.52 & -- -- & -- -- & -- -- & 241 & 230 & 237.80\tabularnewline
16 & -- -- & -- -- & -- -- & 1,781.91 & 1,740.19 & 1,764.31 & -- -- & -- -- & -- -- & 1,970 & 1,951 & 1,959.20\tabularnewline
17 & -- -- & -- -- & -- -- & 13.07 & 12.57 & 12.81 & -- -- & -- -- & -- -- & 397 & 377 & 390.20\tabularnewline
18 & -- -- & -- -- & -- -- & 4.30 & 3.82 & 4.13 & -- -- & -- -- & -- -- & 111 & 108 & 109.60\tabularnewline
19 & -- -- & -- -- & -- -- & 37.71 & 30.72 & 32.32 & -- -- & -- -- & -- -- & 127 & 124 & 125.20\tabularnewline
20 & -- -- & -- -- & -- -- & 60.12 & 57.03 & 59.17 & -- -- & -- -- & -- -- & 434 & 421 & 428.60\tabularnewline
21 & \textbf{1.59} & \textbf{1.55} & \textbf{1.57} & 0.11 & 0.08 & 0.09 & \textbf{25} & \textbf{25} & \textbf{25} & 25 & 25 & 25\tabularnewline
22 & \textbf{1,783.84} & \textbf{1,289.52} & \textbf{1,500.63} & 0.14 & 0.09 & 0.11 & \textbf{65} & \textbf{53} & \textbf{57} & 51 & 46 & 47.80\tabularnewline
23 & -- -- & -- -- & -- -- & 5.40 & 4.99 & 5.20 & -- -- & -- -- & -- -- & 193 & 182 & 188\tabularnewline
24 & -- -- & -- -- & -- -- & 214.81 & 205.24 & 210.35 & -- -- & -- -- & -- -- & 519 & 504 & 511.40\tabularnewline
25 & -- -- & -- -- & -- -- & 1,520.27 & 1,480.51 & 1,495.99 & -- -- & -- -- & -- -- & 867 & 855 & 861.60\tabularnewline
26 & -- -- & -- -- & -- -- & 0.26 & 0.21 & 0.23 & -- -- & -- -- & -- -- & 55 & 52 & 53.40\tabularnewline
27 & -- -- & -- -- & -- -- & 0.56 & 0.49 & 0.53 & -- -- & -- -- & -- -- & 103 & 100 & 101.20\tabularnewline
\hline 
\end{tabular}


==> sut.tex <==
\begin{tabular}{l|l|l|l|l|l}
\hline 
Parameters & $F_1$: Display & $F_2$: Email Viewer & $F_3$: Camera & $F_4$: Video Camera & $F_5$: Video Ringtone\tabularnewline
\hline 
\multirow{3}{*}{Domains} & 0: 16MC & 0: Graphical & 0: 2MP & 0: Yes & 0: Yes\tabularnewline
 & 1: 8MC & 1: Text & 1: 1MP & 1: No & 1: No\tabularnewline
 & 2: BW & 2: None & 2: None &  & \tabularnewline
\hline 
\multirow{14}{*}{Constraints} & \multicolumn{5}{l}{$F_1=0\Rightarrow F_1\neq2$}\tabularnewline
 & \multicolumn{5}{r}{\textbf{Graphical }email viewer requires \textbf{color }display}\tabularnewline
 & \multicolumn{5}{l}{$F_3=0\Rightarrow F_1\neq2$}\tabularnewline
 & \multicolumn{5}{r}{\textbf{2 Megapixel} camera requires \textbf{color} display}\tabularnewline
 & \multicolumn{5}{l}{$F_2=0\Rightarrow F_3\neq0$}\tabularnewline
 & \multicolumn{5}{r}{\textbf{Graphical} email viewer does not support \textbf{2 Megapixel}
camera}\tabularnewline
 & \multicolumn{5}{l}{$F_1=1\Rightarrow F_3\neq0$}\tabularnewline
 & \multicolumn{5}{r}{\textbf{8 Million }color display does not support \textbf{2 Megapixel}
camera}\tabularnewline
 & \multicolumn{5}{l}{$F_4=0\Rightarrow(F_3\neq2\land F_1\neq2)$}\tabularnewline
 & \multicolumn{5}{r}{\textbf{Video camera} requires \textbf{camera} and \textbf{color}
display}\tabularnewline
 & \multicolumn{5}{l}{$F_5=0\Rightarrow F_4=0$}\tabularnewline
 & \multicolumn{5}{r}{\textbf{Video ringtone} cannot occur with NO \textbf{video camera}}\tabularnewline
 & \multicolumn{5}{l}{$\neg(F_1=0\land F_2=1\land F_3=0)$}\tabularnewline
 & \multicolumn{5}{r}{The combination of \textbf{16 Million }colors, \textbf{text }email\textbf{
}viewer and \textbf{2 Megapixel} camera will not be supported}\tabularnewline
\hline 
\end{tabular}

